Dust in the Wind: Composition and Kinematics of Galaxy Outflows at the Peak Epoch of Star Formation

Galactic-scale outflows regulate the stellar mass growth and chemical enrichment of galaxies, yet key outflow properties such as the chemical composition and mass loss rate remain largely unknown. We address these properties with Keck/ESI echellete spectra of nine gravitationally lensed z=2-3 star forming galaxies, probing a range of absorption transitions. Interstellar absorption in our sample is dominated by outflowing material, with typical velocities -150 km/s. Approximately 80% of the total column density is associated with a net outflow. Mass loss rates in the low ionization phase are comparable to or in excess of the star formation rate, with total outflow rates likely higher when accounting for ionized gas. Of order half of the heavy element yield from star formation is ejected in the low ionization phase, confirming that outflows play a critical role in regulating galaxy chemical evolution. Covering fractions vary and are in general non-uniform, with most galaxies having incomplete covering by the low ions across all velocities. Low ion abundance patterns show remarkably little scatter, revealing a distinct "chemical fingerprint" of outflows. Gas phase Si/Fe abundances are significantly super-solar ([Si/Fe]$\gtrsim$0.4) indicating a combination of $\alpha$-enhancement and dust depletion. Derived properties are comparable to the most kinematically broad, metal-rich, and depleted intergalactic absorption systems at similar redshifts, suggesting that these extreme systems are associated with galactic outflows at impact parameters conservatively within a few tens of kpc. We discuss implications of the abundance patterns in z=2-3 galaxies and the role of outflows at this epoch.

==> table_n_ions.tex <==

\begin{deluxetable*}{lcccccccccc}
\tablecolumns{10}
\tablewidth{0pt}
\tablecaption{Ion column densities\label{tab:transitions}}

\tablehead{
\colhead{Ion} & \colhead{CSWA 141} & \colhead{CSWA 103} & \colhead{CSWA 19} & \colhead{CSWA 40} & \colhead{CSWA 2} & \colhead{CSWA 128} & \colhead{CSWA 164} & \colhead{CSWA 39} & \colhead{CSWA 38} \\
\colhead{$\Delta$v [\kms]} & \colhead{-400 $-$ -150} & \colhead{-500 $-$ 0} & \colhead{-250 $-$ 0} & \colhead{-250 $-$ 50} & \colhead{-200 $-$ 300} & \colhead{-300 $-$ 100} & \colhead{-400 $-$ 150} & \colhead{-300 $-$ 0} & \colhead{-400 $-$ 0} \\
}

\medskip
\startdata

H I 1216\tablenotemark{a} &  --  & 21.15$_{-1.98}^{+0.47}$ &  --  &  --  &  --  & 21.56$_{-0.43}^{+0.20}$ & 20.34$_{-0.33}^{+0.23}$ & 20.63$_{-0.34}^{+0.79}$ & 20.57$_{-0.11}^{+0.30}$  \\



\enddata
\tablenotetext{}{All column densities are in units of $10^{14}$ cm$^{-2}$ and are integrated over the velocity range $\Delta$v, except where noted otherwise.}
\tablenotetext{a}{H I column densities are given as $\log N$, with $N$ in units of cm$^{-2}$.}
\tablenotetext{b}{Lower limit corresponding to optical depth $\tau > 2$.}
\tablenotetext{c}{2$\sigma$ upper limit.}

\end{deluxetable*}

